Fast Global Convergence of Natural Policy Gradient Methods with Entropy Regularization

Natural policy gradient (NPG) methods are among the most widely used policy optimization algorithms in contemporary reinforcement learning. This class of methods is often applied in conjunction with entropy regularization -- an algorithmic scheme that encourages exploration -- and is closely related to soft policy iteration and trust region policy optimization. Despite the empirical success, the theoretical underpinnings for NPG methods remain limited even for the tabular setting. This paper develops $\textit{non-asymptotic}$ convergence guarantees for entropy-regularized NPG methods under softmax parameterization, focusing on discounted Markov decision processes (MDPs). Assuming access to exact policy evaluation, we demonstrate that the algorithm converges linearly -- or even quadratically once it enters a local region around the optimal policy -- when computing optimal value functions of the regularized MDP. Moreover, the algorithm is provably stable vis-\`a-vis inexactness of policy evaluation. Our convergence results accommodate a wide range of learning rates, and shed light upon the role of entropy regularization in enabling fast convergence.

==> pf-thm-perturb.tex <==
\section{Proof of Theorem \ref{thm:SPI-perturbed}}
\label{Sec:Pfthmperturb}

For notational convenience, 
we denote by $V_{\tau,\mathrm{p}}^{\pi}$ (resp.~$V_{\mathrm{p}}^{\pi}$)
the regularized (resp.~unregularized) value function of policy $\pi$
in $\mathcal{M}_{\mathrm{p}}$. 
% The notation $V_{\mathrm{p}}^{\pi}$ (resp.~$Q_{\mathrm{p}}^{\pi}$) represents the unregularized value function (resp.~Q-function) of policy $\pi$ in $\mathcal{M}_{\mathrm{p}}$. 
Let $V_{\tau,\mathrm{p}}^{\star}$
indicate the optimal entropy-regularized value function for $\mathcal{M}_{\mathrm{p}}$,
with $\pi_{\tau,\mathrm{p}}^{\star}$ denoting the corresponding optimal
policy. We shall also let $\mu_{\tau,\mathrm{p}}^{\star}$ represent the stationary
distribution of $\mathcal{M}_{\mathrm{p}}$ under the optimal policy
$\pi_{\tau,\mathrm{p}}^{\star}$. 
%For any policy iterate $\pi^{(t)}$, we let $Q_{\tau,\mathrm{p}}^{(t)}:=Q_{\tau,\mathrm{p}}^{\pi^{(t)}}$ (resp.~$Q_{\tau}^{(t)}:=Q_{\tau}^{\pi^{(t)}}$) represent the regularized Q-function of policy $\pi^{(t)}$ in $\mathcal{M}_{\mathrm{p}}$ (resp.~$\mathcal{M}$). 
%
Before proceeding, we record several facts about $\mathcal{M}_{\mathrm{p}}$ that prove useful. 
%
\begin{lemma}
\label{lem:useful-facts-Mperturbed}
The auxiliary MDP $\mathcal{M}_{\mathrm{p}}=(\mathcal{S},\mathcal{A},P_{\mathrm{p}},r,\gamma)$ with $P_{\mathrm{p}}$ defined in \eqref{eq:perturbed-transition} satisfies:
%
\begin{enumerate}
\item For any distribution $\rho$ and any policy $\pi$, one has 
\begin{subequations}
%
\begin{align}
	0\leq V_{\tau,\mathrm{p}}^{\pi}\big(\rho \big)\leq \frac{1+\tau\log|\mathcal{A}|}{1-\gamma}.
	\label{eq:V-perturb-range}
\end{align}
%
\item The stationary distribution $\mu_{\tau,\mathrm{p}}^{\star}(s)$ of $\mathcal{M}_{\mathrm{p}}$ under policy $\pi_{\tau,\mathrm{p}}^{\star}$ obeys
%
\begin{align}
	\min_{s\in\mathcal{S}}\mu_{\tau,\mathrm{p}}^{\star}(s)\geq \xi / |\mathcal{S}|.
	\label{eq:min-mu-perturb}
\end{align}
%
\item For any policy $\pi$, one has
%
\begin{align}
	& \big\| V^{\pi}_\tau - V_{\tau,\mathrm{p}}^{\pi} \big\|_{\infty}  \leq  \frac{2\xi \gamma (1+\tau\log|\mathcal{A}|)}{(1-\gamma)^{2}} ,
	\qquad
	%\quad \text{and} \quad
	\left\Vert Q_{\tau,\mathrm{p}}^{\pi}-Q_{\tau}^{\pi}\right\Vert _{\infty}  
	\leq \frac{2\xi \gamma (1+\tau\log|\mathcal{A}|)}{(1-\gamma)^{2}}
	\label{eq:V-Vp-diff} \\
	& \qquad \qquad \text{and} \qquad \big\| V_{\tau,\mathrm{p}}^{\pi}-V^{\pi}\big\|_{\infty} \leq\frac{\tau\log|\mathcal{A}|}{1-\gamma} + \frac{2\xi \gamma (1+\tau\log|\mathcal{A}|)}{(1-\gamma)^{2}}.
	\label{eq:V-Vp-diff-true}
\end{align}
%
\end{subequations}
\end{enumerate}
\end{lemma}



%%\[
%\forall s\in\mathcal{S}:\qquad\pi^{(t+1)}(\cdot|s)\,\propto\,\exp\left(Q_{\tau}^{(t)}(s,\cdot)/\tau\right).
%\]

%Here, $\delta >0$ is a quantity that, in view of \eqref{eq:V-Vp-diff} in Lemma~\ref{lem:useful-facts-Mperturbed}, can be taken as $\delta = \frac{2\xi \gamma (1+\tau\log|\mathcal{A}|)}{(1-\gamma)^{2}}$. 
%By comparing this with the form (\ref{eq:soft_greedy_approximate})

The proof of the above lemma can be found in Appendix~\ref{proof:lem:useful-facts-Mperturbed}. We are now in a position to prove Theorem \ref{thm:SPI-perturbed}. 
Invoking Theorem \ref{thm:spi} yields that
%
\begin{align}
	V_{\tau,\mathrm{p}}^{\star}(\rho)-V_{\tau,\mathrm{p}}^{(t)}(\rho)\leq {\epsilon}/{2}
	\label{eq:Vp-tau-UB1}
\end{align}
%
as soon as 
\[
t\geq T_{\mathrm{p}}:=\frac{1}{1-\gamma}\log\left(2\Bigg\|\frac{\rho}{\mu_{\tau,\mathrm{p}}^{\star}}\Bigg\|_{\infty}\frac{V_{\tau,\mathrm{p}}^{\star}\big(\mu_{\tau,\mathrm{p}}^{\star}\big)-V_{\tau,\mathrm{p}}^{(0)}\big(\mu_{\tau,\mathrm{p}}^{\star}\big)}{\epsilon}\right).
\]
%
The next step is to develop a cleaner upper bound on $T_{\mathrm{p}}$. Towards
this, we observe that
%
\begin{align}
	T_{\mathrm{p}} & \overset{\mathrm{(i)}}{\leq} \frac{1}{1-\gamma}\log\left(2\Bigg\|\frac{1}{\mu_{\tau,\mathrm{p}}^{\star}}\Bigg\|_{\infty}\frac{1+\tau\log|\mathcal{A}|}{ (1-\gamma) \epsilon}\right) 
 		 \overset{\mathrm{(ii)}}{\leq} \frac{1}{1-\gamma}\log\left(4\Bigg\|\frac{1}{\mu_{\tau,\mathrm{p}}^{\star}}\Bigg\|_{\infty}\frac{1}{(1-\gamma)\epsilon}\right) \notag\\
	& \overset{\mathrm{(iii)}}{\leq} \frac{1}{1-\gamma}\log\left(\frac{4|\mathcal{S}|}{\xi(1-\gamma)\epsilon}\right) . 
	\label{eq:Tp-UB1}
\end{align}
%
Here, (i) arises from the trivial bound $\rho \leq 1$ as well as the inequality \eqref{eq:V-perturb-range}, (ii) follows from the choice $\tau \leq \frac{(1-\gamma)\epsilon}{\log |\mathcal{A}|}$ and the range $0<\epsilon \le \frac{1}{1-\gamma}$, while (iii) results from the inequality \eqref{eq:min-mu-perturb}. 



Additionally,  it is straightforward to derive from the inequality \eqref{eq:V-Vp-diff-true} that
%
\begin{align*}
\left|V^{\star}(\rho)-V_{\tau,\mathrm{p}}^{\star}(\rho)\right| 
&= \max \left\{V^{\star}(\rho)- V_{\tau,\mathrm{p}}^{\pi^\star}(\rho) +V_{\tau,\mathrm{p}}^{\pi^\star}(\rho) - V_{\tau,\mathrm{p}}^{\star}(\rho), 
~V_{\tau,\mathrm{p}}^{\star}(\rho) - V^{\pi^\star_{\tau,\mathrm{p}}}(\rho) + V^{\pi^\star_{\tau,\mathrm{p}}}(\rho) - V^{\star}(\rho) \right\}\\
	&\stackrel{\mathrm{(i)}}{\leq}
\max \left\{V^{\star}(\rho)- V_{\tau,\mathrm{p}}^{\pi^\star}(\rho), 
~V_{\tau,\mathrm{p}}^{\star}(\rho) - V^{\pi^\star_{\tau,\mathrm{p}}}(\rho) \right\} \\
%
& \leq \frac{\tau\log|\mathcal{A}|}{1-\gamma}+\frac{2\xi\gamma(1+\tau\log|\mathcal{A}|)}{(1-\gamma)^{2}} \leq \frac{\tau\log|\mathcal{A}|}{1-\gamma}+\frac{4\xi\gamma}{(1-\gamma)^{2}} ,
\end{align*}
where the optimality of $\pi^{\star}$ (resp.~$\pi^\star_{\tau,\mathrm{p}}$) w.r.t.~$V$ (resp.~$V_{\tau}$) is invoked in (i), and the last inequality holds if $\tau \leq \frac{(1-\gamma)\epsilon}{\log |\mathcal{A}|}$. Likewise, the inequality \eqref{eq:V-Vp-diff-true} also implies that
%
\begin{align*}
	\left|V^{\pi^{(t)}}(\rho)-V_{\tau,\mathrm{p}}^{(t)}(\rho)\right| 
	& \leq \frac{\tau\log|\mathcal{A}|}{1-\gamma}+\frac{4\xi\gamma}{(1-\gamma)^{2}}
\end{align*}
%
for any distribution $\rho$, with the proviso that $\tau \leq \frac{(1-\gamma)\epsilon}{\log |\mathcal{A}|}$. These taken collectively with \eqref{eq:Vp-tau-UB1} lead to
%
\begin{align}
V^{\star}(\rho)-V^{\pi^{(t)}}(\rho) & \leq V_{\tau,\mathrm{p}}^{\star}(\rho)-V_{\tau,\mathrm{p}}^{(t)}(\rho)+\left|V^{\star}(\rho)-V_{\tau,\mathrm{p}}^{\star}(\rho)\right|+\left|V^{\pi^{(t)}}(\rho)-V_{\tau,\mathrm{p}}^{(t)}(\rho)\right|\nonumber \\
 & \leq\frac{\epsilon}{2} +\frac{2\tau\log|\mathcal{A}|}{1-\gamma}+\frac{8\xi}{(1-\gamma)^{2}}.
	\label{eq:Vbound-1234}
\end{align}
%
% where the last line follows from the inequality \eqref{eq:min-mu-perturb} in Lemma~\ref{lem:useful-facts-Mperturbed}.
Taking $\tau=\frac{(1-\gamma)\epsilon}{8\log|\mathcal{A}|}$ and $\xi=\frac{\epsilon^2(1-\gamma)^{5}}{50|\cS|^2}$
thus guarantees that
%
\begin{align*}
	V^{\star}(\rho)-V^{\pi^{(t)}}(\rho)  
  	<\frac{\epsilon}{2} + \frac{\epsilon}{4} + \frac{\epsilon}{4} = \epsilon.
	% \label{eq:Vbound-12345}
\end{align*}
%
Furthermore, the above choices of $\xi$ allows us to upper bound \eqref{eq:Tp-UB1} by
%
%
\begin{align}
	T_{\mathrm{p}} & \leq \frac{1}{1-\gamma}\log\left(\frac{4|\mathcal{S}|}{\xi(1-\gamma)\epsilon}\right) 
	\le \frac{1}{1-\gamma}\log\left(\frac{200|\mathcal{S}|^3}{(1-\gamma)^{6}\epsilon^{3}}\right)
	< \frac{3}{1-\gamma}\log\left(\frac{6|\mathcal{S}|}{(1-\gamma)^2\epsilon}\right).
	\label{eq:Tp-UB2}
\end{align}
%
Finally, by replacing $\rho$ with a singleton distribution for each $s\in \cS$, we 
conclude the proof. 



==> reduction.tex <==
\section{An adaptive approach to solve the original MDP} \label{sec:reduction}

As has been discussed, simply plugging in the choice of $\tau = \frac{(1-\gamma)\epsilon}{4\log|\mathcal{A}|}$ leads to an iteration complexity of $O\left(\frac{\log|\mathcal{A}|}{(1-\gamma) \epsilon \eta}\log\left(\frac{1}{\epsilon}\right)\right)$. Inspired by the standard reduction techniques in the optimization literature (see also \cite{yang2020finding}), we seek to adaptively decrease $\tau$ to the desired level, which leads to Algorithm \ref{alg:dacong-reduction}. The algorithm halves $\tau$ after every call of Algorithm \ref{alg:entropy-npg} and set $\pi^{(0)}_{i+1}(a|s) \propto {\pi}^{(T+1)}_{i}(a|s)^2$ in response to the change of $\tau$. We show that Algorithm \ref{alg:dacong-reduction} needs no more than $O\prn{\log \frac{\log |\mathcal{A}|}{(1-\gamma)\epsilon}}$ reduction rounds, or $O\prn{\frac{\log|\mathcal{A}|}{(1-\gamma)\eta \epsilon }\log \frac{1}{1-\gamma}}$ NPG iterations in total to find an $\epsilon$-optimal policy for the original unregularized MDP, thus allowing us to shave off the extra $\log (1/\epsilon)$ factor in the iteration complexity without adaptation.  



\begin{algorithm}[ht]
	\DontPrintSemicolon
	   \textbf{inputs:} learning rate $0< \eta\leq 1-\gamma$. \\
		% number of iterations $T$, 
	  \textbf{initialization:} $\tau_0 = 1$, $\plcy_{0}^{(0)}(a|s) = 1/|\mathcal{A}|, \forall (s,a)\in\mathcal{S}\times\mathcal{A}$ is the uniform poicy. \\
	
	
	   \For{$i=0,1,2,\cdots$}
		{
			Call Algorithm \ref{alg:entropy-npg} with entropy regularization parameter $\tau_i$, step size $\eta$ and initialization $\pi^{(0)}_{i}$ and get ${\pi}^{(T_i+1)}_{i}$ with $T_i = \lceil {\frac{1}{\eta\tau_i}\log\frac{8}{1-\gamma}} \rceil$, where $\lceil \cdot \rceil$ is the ceiling function. \\
			Set $\pi^{(0)}_{i+1}(a|s) \propto {\pi}^{(T_i+1)}_{i}(a|s)^2$ and
			$\tau_{i+1} = \tau_{i}/2$.
		}
	
	   %\textbf{return:} ${Q}_{T}$. 
		\caption{Adaptive entropy regularization to solve the original MDP}
	 \label{alg:dacong-reduction}
	\end{algorithm}
 
 For notation simplicity, we use $Q^\star_{i}$ to denote $Q^\star_{\tau_i}$, i.e. the optimal Q-function with the regularization parameter $\tau_i$. We use $\pi_{i}^{(t)}$ to denote the $t$-th policy in the $i$-th reduction round and write its associated $Q$ function as $Q_{i}^{(t)}$, and the auxiliary sequence as $\xi_{i}^{(t)}$, where the latter is defined similar to \eqref{defn:xi-t-sequence} as follows:
 \begin{subequations}
	\begin{align}
		\xi_{0}^{(0)}(\s, \ac) &:= 1,\\
		\xi_{i+1}^{(0)}(\s, \ac) &:= \xi_{i}^{(T+1)}(\s, \ac)^2, \label{eq:xi_squared_trick}\\
		\xi_{i}^{(t+1)}(s,a) &:= \big[ \xi_{i}^{(t)}(s,a) \big]^{\alpha_i} \exp\prnBig{\prn{1-\alpha_i}\frac{Q_{i}^{(t)} (s,a)}{\tau} }.,
	\end{align}	
\end{subequations}
where $\alpha_i := 1 - \frac{\eta \tau_i}{1 - \disct}$. As before,	 $\pi_{i}^{(t)}(\cdot|s) \propto \xi_{i}^{(t)}(s, \cdot)$ hold for all $s\in\mathcal{S}$ and $i, t \ge 0$. We also have the following claim regarding the optimal soft $Q$-functions with different regularization parameters. 
\begin{claim}\label{claim:reduction}
	For any $\tau, \tau' > 0$, we have
	\begin{equation}\label{eq:reduction-Q}
	\norm{Q_{\tau'}^\star - Q_{\tau}^\star}_\infty \le \frac{|\tau-\tau'|\log|\mathcal{A}|}{1-\gamma}.
	\end{equation}
\end{claim}

With this claim, it is straightforward to see that
\begin{align}\label{eq:reduction_triangle}
\normbig{{Q}^\star - {Q}^{\pi_{i}^{(T_{i}+1)}}}_\infty &\le 	\normbig{{Q}^\star - {Q}_i^{\star}}_\infty  + \normbig{{Q}_i^{(T_{i}+1)} - {Q}^{\pi_{i}^{(T_{i}+1)}}}_\infty+ \normbig{{Q}_{i}^\star - {Q}_{i}^{(T_{i}+1)}}_\infty  \notag \\ 
&\leq \frac{2\tau_{i}\log |\cA|}{1-\gamma} + \normbig{{Q}_{i}^\star - {Q}_{i}^{(T_{i}+1)}}_\infty  ,
\end{align}
where it boils down to control the second term.
From our analysis in Section~\ref{Sec:pfNPG-eta} (cf. \eqref{eq:xtplus1-recursion-bound}), the following inequalities hold for each reduction round:
	\begin{equation} \label{eq:reduction-contraction}
		\begin{bmatrix}
			\normbig{{Q}_{i}^\star - {Q}_{i}^{(T_i+1)}}_\infty \\[1ex]
			\normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(T_i+1)}}_\infty 
			\end{bmatrix}  \le  (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \right\} \begin{bmatrix}
	\disct \\
	1
	\end{bmatrix}.
	\end{equation}

In addition, we have
	\begin{align} \label{eq:reduction-Q-gap}
		\normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty \le \frac{\tau_{i}\gamma}{1-\gamma}{\norm{\log\pi_{i}^{(0)}-\log\pi_{i}^\star}}_\infty \le \frac{2\gamma}{1-\gamma}{\norm{Q_{i}^\star - \tau_{i}\log\xi^{(0)}_{i}}}_\infty,
	\end{align}
	where the first step results from \cite[Lemma 24]{mei2020global} that for any policy $\pi$ and regularization parameter $\tau$,
		\[
		V_\tau^\star(\rho) - V_\tau^\pi(\rho) = \frac{\tau}{1-\gamma}\exlim{s\sim d_\rho^\pi}{\KL \prn{\pi(\cdot|s)\,\|\,\pi_\tau^\star(\cdot|s)}} \leq  \frac{\tau}{1-\gamma}{\norm{\log\pi-\log\pi_\tau^\star}}_\infty,
	\]
	and the second step is due to \eqref{eq:log_pi_diff}.
	
Putting \eqref{eq:reduction-contraction} and \eqref{eq:reduction-Q-gap} together, we obtain
	\begin{align*}
		\normbig{{Q}_{i+1}^\star - \tau_{i+1} \log \xi_{i+1}^{(0)}}_\infty &= \normbig{{Q}_{i+1}^\star - \tau_{i} \log \xi_{i}^{(T+1)}}_\infty \\
		&\le \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(T+1)}}_\infty + \normbig{{Q}_{i+1}^\star - {Q}_{i}^\star}_\infty\\
		&\le \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(T+1)}}_\infty + \frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma} \\
		& \le (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \right\} + \frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma} \notag \\
		&  \le (1 - \eta \tau_{i})^{T_{i}} \frac{2}{1-\gamma}\normbig{{Q}_{i}^\star - \tau_i \log \xi_{i}^{(0)}}_\infty + \frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma},
	\end{align*}
	where the first line follows from \eqref{eq:xi_squared_trick}, and the third line is due to \eqref{eq:reduction-Q}. Since $\normbig{{Q}_{0}^\star - \tau_{0} \log \xi_{0}^{(0)}}_\infty = \normbig{{Q}_{0}^\star}_\infty \le \frac{1}{1-\gamma} + \frac{\tau_0\log|\mathcal{A}|}{1-\gamma}\le 2\frac{\tau_{0}\log|\mathcal{A}|}{1-\gamma}$, from the above inequality, we have  
	\begin{equation}
	\normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \le 2\frac{\tau_{i}\log|\mathcal{A}|}{1-\gamma}
 \end{equation}
holds for all $i\ge0$ by induction, as long as $T_{i} = \lceil {\frac{1}{\eta\tau_{i}}\log\frac{8}{1-\gamma}} \rceil $. Plugging back to \eqref{eq:reduction-contraction}, we obtain 
	\begin{align*}
			\normbig{{Q}_{i}^\star - {Q}_{i}^{(T_i+1)}}_\infty 
			  &\le (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \right\} \gamma \\
			&\le\frac{\tau_{i}\log|\mathcal{A}|}{1-\gamma}.
	\end{align*}
Plugging it back to \eqref{eq:reduction_triangle} leads to
 \[
		\normbig{{Q}^\star - {Q}^{\pi_{i}^{(T_{i}+1)}}}_\infty \le \frac{2\tau_{i}\log |\cA|}{1-\gamma} + \normbig{{Q}_{i}^\star - {Q}_{i}^{(T_{i}+1)}}_\infty \le \frac{3\tau_{i}\log |\cA|}{1-\gamma} \le \epsilon.
\]
The last inequality holds as long as $\tau_{i+1} \le \frac{(1-\gamma) \epsilon}{4\log|\mathcal{A}|}$, which is achieved with at most $S :=O\prn{\log \frac{\log |\mathcal{A}|}{(1-\gamma)\epsilon}}$ reduction rounds of Algorithm \ref{alg:dacong-reduction}, and a total of 
	\[
		\sum_{i=0}^{S} T_{i} \le 2 T_{S}= O\prn{\frac{\log|\mathcal{A}|}{(1-\gamma)\eta \epsilon }\log \frac{1}{1-\gamma}}
	\] iterations to find an $\epsilon$-optimal policy for the original MDP.
	
 
%	\begin{theorem}
%		For any learning rate $0 < \eta \le 1-\gamma$, Algorithm \ref{alg:dacong-reduction} satisfies
%		\begin{align}
%				\normbig{{Q}_{i+1}^\star - \tau_{i+1} \log \xi_{i+1}^{(0)}}_\infty 
%				& \le   (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i\normbig{{Q}_{i}^\star - \tau_i \log \xi_{i}^{(0)}}_\infty \right\}+ \frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma},\label{eqn:reduction-1}\\
%				 \normbig{{Q}_{i+1}^\star - {Q}_{i+1}^{(0)}}_\infty & \le  \frac{2\gamma}{1-\gamma}{\norm{Q_{i+1}^\star - \tau_{i+1}\log\xi^{(0)}_{i+1}}}_\infty,\label{eqn:reduction-2}\\
%				 \normbig{{Q}_{i}^\star - {Q}_{i}^{(T_i+1)}}_\infty 
%				& \le (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \right\} \gamma 
%		\end{align}
%		for all $i\ge 0$.
%		\label{thm:reduction}
%	\end{theorem}

%	The theorem implies that when we have $\normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \le 2\frac{\tau_{i}\log|\mathcal{A}|}{1-\gamma}$, it suffices to set $T_{i} = {\frac{1}{\eta\tau_{i}}\log\frac{8}{1-\gamma}}$ to get
%	\[
%		\normbig{{Q}_{i+1}^\star - \tau_{i+1} \log \xi_{i+1}^{(0)}}_\infty \le (1 - \eta \tau_{i})^{T_{i}} \frac{2}{1-\gamma}\normbig{{Q}_{i}^\star - \tau \log \xi_{i}^{(0)}}_\infty + \frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma} \le 2\frac{\tau_{i+1}\log|\mathcal{A}|}{1-\gamma}.
%	\]


%	Note that we also get
%	\begin{align*}
%			\normbig{{Q}_{i}^\star - {Q}_{i}^{(T_i+1)}}_\infty 
%			  &\le (1 - \eta \tau_{i})^{T_{i}}  \left\{ \normbig{{Q}_{i}^\star - {Q}_{i}^{(0)}}_\infty +  2\alpha_i \normbig{{Q}_{i}^\star - \tau_{i} \log \xi_{i}^{(0)}}_\infty \right\} \gamma \\
%			&\le\frac{\tau_{i}\log|\mathcal{A}|}{1-\gamma}.
%	\end{align*}
%	As long as $\tau_{i+1} \le \frac{(1-\gamma) \epsilon}{4\log|\mathcal{A}|}$, we have
%	\[
%		\normbig{{Q}^\star - {Q}^{\pi_{i}^{(T_{i}+1)}}}_\infty \le \frac{2\tau_{i}\log |\cA|}{1-\gamma} + \normbig{{Q}_{i}^\star - {Q}_{i}^{(T_{i}+1)}}_\infty \le \frac{3\tau_{i}\log |\cA|}{1-\gamma} \le \epsilon.
%	\]





\begin{proof}[Proof of Claim~\ref{claim:reduction}]
For any $(s,a) \in \mathcal{S}\times \mathcal{A}$, we have
	\begin{align*}
		Q_\tau^\star(s, a) = Q_\tau^{\pi_\tau^\star}(s, a) \ge Q_\tau^{\pi_{\tau'}^\star}(s, a) \ge Q_{\tau'}^{\pi_{\tau'}^\star}(s, a) - \frac{|\tau-\tau'|\log|\mathcal{A}|}{1-\gamma} = Q_{\tau'}^\star(s, a) - \frac{|\tau-\tau'|\log|\mathcal{A}|}{1-\gamma}.
	\end{align*}
%	Similarly, we have
%	\begin{align*}
%		Q_{\tau'}^\star(s, a) \ge Q_{\tau}^\star(s, a) - \frac{|\tau-\tau'|\log|\mathcal{A}|}{1-\gamma}.
%	\end{align*}
Swapping $\tau$ and $\tau'$ obtains the other direction by symmetry. The proof is complete. 
\end{proof}



